Toward Self-Improvement of LLMs via Imagination, Searching, and Criticizing

Despite the impressive capabilities of Large Language Models (LLMs) on various tasks, they still struggle with scenarios that involves complex reasoning and planning. Recent work proposed advanced prompting techniques and the necessity of fine-tuning with high-quality data to augment LLMs' reasoning abilities. However, these approaches are inherently constrained by data availability and quality. In light of this, self-correction and self-learning emerge as viable solutions, employing strategies that allow LLMs to refine their outputs and learn from self-assessed rewards. Yet, the efficacy of LLMs in self-refining its response, particularly in complex reasoning and planning task, remains dubious. In this paper, we introduce AlphaLLM for the self-improvements of LLMs, which integrates Monte Carlo Tree Search (MCTS) with LLMs to establish a self-improving loop, thereby enhancing the capabilities of LLMs without additional annotations. Drawing inspiration from the success of AlphaGo, AlphaLLM addresses the unique challenges of combining MCTS with LLM for self-improvement, including data scarcity, the vastness search spaces of language tasks, and the subjective nature of feedback in language tasks. AlphaLLM is comprised of prompt synthesis component, an efficient MCTS approach tailored for language tasks, and a trio of critic models for precise feedback. Our experimental results in mathematical reasoning tasks demonstrate that AlphaLLM significantly enhances the performance of LLMs without additional annotations, showing the potential for self-improvement in LLMs.

==> floats/figure_ablation_mcts.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.75\textwidth]{figures/mcts_ablation.png}
    \caption{Ablation study on the GSM8K test set of various enhancements to the proposed efficient MCTS, including \prm{}, fastrollout with \orm{}, state merging, and increasing the number of rollouts.}
    \label{fig:search_ablation}
\end{figure}


% \begin{figure}[ht]
%     \centering
%     % Minipage for the Table
%     \begin{minipage}{0.25\textwidth}
%         \centering
%         \begin{tabular}{|l|c|}
%             \hline
%             Column 1 & Column 2 \\
%             \hline
%             Item 1 & Item 2 \\
%             Item 3 & Item 4 \\
%             \hline
%         \end{tabular}
%         \caption{Example Table}
%         \label{table:example_table}
%     \end{minipage}
%     \hfill
%     % Minipage for the Figure
%     \begin{minipage}{0.7\textwidth}
%         \centering
%         \includegraphics[width=0.9\textwidth]{figures/mcts_ablation.png}
%     \caption{Ablation study on the GSM8K test set of various enhancements to the proposed efficient MCTS, including \prm{}, fastrollout with \orm{}, state merging, and increasing the number of rollouts.}
%     \label{fig:search_ablation}
%     \end{minipage}
% \end{figure}


==> floats/table_ablation_mcts.tex <==
% 2) ablation study:
% search times, each components

\begin{table}[!htb]
    \centering
    \begin{tabular}{cl|c}
        \multicolumn{2}{c|}{Method}         & GSM8K \\
        \hline
        \multicolumn{2}{l|}{MCTS}           & $84.9$ \\
        \hline
           & + Step reward                  & $85.9$ \\
           & ~~+ Fast-rollout               & $86.5$ \\
           & ~~~~+ State merge              & $87.0$ \\
           & ~~~~~~+ Large $r=230$          & $88.9$ \\
        \hline
    \end{tabular}
    \vspace{4mm}
    \caption{Ablation study over GSM8K test set.}
    \label{tab:ablation_result}
\end{table}

